Language-Driven Visual Consensus for Zero-Shot Semantic Segmentation

The pre-trained vision-language model, exemplified by CLIP, advances zero-shot semantic segmentation by aligning visual features with class embeddings through a transformer decoder to generate semantic masks. Despite its effectiveness, prevailing methods within this paradigm encounter challenges, including overfitting on seen classes and small fragmentation in masks. To mitigate these issues, we propose a Language-Driven Visual Consensus (LDVC) approach, fostering improved alignment of semantic and visual information.Specifically, we leverage class embeddings as anchors due to their discrete and abstract nature, steering vision features toward class embeddings. Moreover, to circumvent noisy alignments from the vision part due to its redundant nature, we introduce route attention into self-attention for finding visual consensus, thereby enhancing semantic consistency within the same object. Equipped with a vision-language prompting strategy, our approach significantly boosts the generalization capacity of segmentation models for unseen classes. Experimental results underscore the effectiveness of our approach, showcasing mIoU gains of 4.5 on the PASCAL VOC 2012 and 3.6 on the COCO-Stuff 164k for unseen classes compared with the state-of-the-art methods.

==> cvpr_sections/experiment.bak.tex <==
\section{Experiment}
\begin{table*}[!t]
\centering
\resizebox{0.99\linewidth}{!}{%
\setlength{\tabcolsep}{0.7em}
    {\renewcommand{\arraystretch}{1.1}
\begin{tabular}{cc|cl|cccc|cccc}
\toprule
\multicolumn{2}{l|}{}  &\multicolumn{1}{l|}{\multirow{2}{*}{Pipeline}}      & \multicolumn{4}{c|}{\textbf{PASCAL VOC 2012}} &\multicolumn{4}{c}{\textbf{COCO-Stuff 164k}}
\\ \cline{4-11} 

\multicolumn{2}{l|}{}  & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{pAcc}            & \multicolumn{1}{c|}{mIoU(S)}          & \multicolumn{1}{c|}{\textbf{mIoU(U)}} &\multicolumn{1}{c|}{hIoU}& \multicolumn{1}{c|}{pAcc}            & \multicolumn{1}{c|}{mIoU(S)}          & \multicolumn{1}{c|}{\textbf{mIoU(U)}} &\multicolumn{1}{c}{hIoU}\\ \hline

\multicolumn{2}{l|}{SPNet~\cite{xian2019semantic}}  & \multicolumn{1}{l|}{One-Stage}     & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ 78.0 } & \multicolumn{1}{c|}{ 15.6 } & \multicolumn{1}{c|}{ 26.1 } & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ 35.2 } & \multicolumn{1}{c|}{ 8.7 } & \multicolumn{1}{c}{ 14.0 }         \\

\multicolumn{2}{l|}{ZS3~\cite{bucher2019zero}}  & \multicolumn{1}{l|}{One-Stage}     & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ 77.3 } & \multicolumn{1}{c|}{ 17.7 } & \multicolumn{1}{c|}{ 28.7 } & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ 34.7 } & \multicolumn{1}{c|}{ 9.5 } & \multicolumn{1}{c}{ 15.0 }         \\ 

\multicolumn{2}{l|}{CaGNet~\cite{gu2020context}}  & \multicolumn{1}{l|}{One-Stage}     & \multicolumn{1}{c|}{ 80.7 } & \multicolumn{1}{c|}{ 78.4 } & \multicolumn{1}{c|}{ 26.6 } & \multicolumn{1}{c|}{ 39.7 } & \multicolumn{1}{c|}{ 56.6 } & \multicolumn{1}{c|}{ 33.5 } & \multicolumn{1}{c|}{ 12.2 } & \multicolumn{1}{c}{ 18.2 }         \\ 

\multicolumn{2}{l|}{SIGN~\cite{cheng2021sign}} & \multicolumn{1}{l|}{One-Stage}     & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ 75.4 } & \multicolumn{1}{c|}{ 28.9 } & \multicolumn{1}{c|}{ 41.7 } & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ 32.3 } & \multicolumn{1}{c|}{ 15.5 } & \multicolumn{1}{c}{ 20.9 }         \\ 

\multicolumn{2}{l|}{STRICT~\cite{pastore2021closer}}  & \multicolumn{1}{l|}{One-Stage}     & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ 82.7 } & \multicolumn{1}{c|}{ 35.6 } & \multicolumn{1}{c|}{ 49.8 } & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ 35.3 } & \multicolumn{1}{c|}{ 30.3 } & \multicolumn{1}{c}{ 32.6 }         \\

\multicolumn{2}{l|}{ZegFormer~\cite{ding2022decoupling}}  & \multicolumn{1}{l|}{Two-Stage}     & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ 86.4 } & \multicolumn{1}{c|}{ 63.6 } & \multicolumn{1}{c|}{ 73.3 } & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ 36.6 } & \multicolumn{1}{c|}{ 33.2 } & \multicolumn{1}{c}{ 34.8 }         \\

\multicolumn{2}{l|}{Zsseg~\cite{xu2022simple}}  & \multicolumn{1}{l|}{Two-Stage}     & \multicolumn{1}{c|}{ 90.0 } & \multicolumn{1}{c|}{ 83.5 } & \multicolumn{1}{c|}{ 72.5 } & \multicolumn{1}{c|}{ 77.5 } & \multicolumn{1}{c|}{ 60.3 } & \multicolumn{1}{c|}{ 39.3 } & \multicolumn{1}{c|}{ 36.3 } & \multicolumn{1}{c}{ 37.8 }         \\

\multicolumn{2}{l|}{DeOP~\cite{han2023zero}}  & \multicolumn{1}{l|}{One-Stage}     & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ 88.2 } & \multicolumn{1}{c|}{ 74.6 } & \multicolumn{1}{c|}{ 80.8 } & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ 38.0 } & \multicolumn{1}{c|}{ 38.4 } & \multicolumn{1}{c}{ 38.2 }         \\

\multicolumn{2}{l|}{ZegCLIP~\cite{zhou2022zegclip}}  & \multicolumn{1}{l|}{One-Stage}     & \multicolumn{1}{c|}{ 94.6 } & \multicolumn{1}{c|}{ 91.9 } & \multicolumn{1}{c|}{ 77.8 } & \multicolumn{1}{c|}{ 84.3 } & \multicolumn{1}{c|}{ 62.0 } & \multicolumn{1}{c|}{ 40.2 } & \multicolumn{1}{c|}{ 41.4 } & \multicolumn{1}{c}{ 40.8 } \\ \hline

\multicolumn{2}{l|}{SCVR(Ours)}   & \multicolumn{1}{l|}{One-Stage}     & \multicolumn{1}{c|}{ \textbf{95.5} } & \multicolumn{1}{c|}{ \textbf{92.5} } & \multicolumn{1}{c|}{ \textbf{82.3} } & \multicolumn{1}{c|}{ \textbf{87.2} } & \multicolumn{1}{c|}{ \textbf{64.3} } & \multicolumn{1}{c|}{ \textbf{43.2} } & \multicolumn{1}{c|}{ \textbf{45.0} } & \multicolumn{1}{c}{ \textbf{44.1} } \\ \bottomrule
\end{tabular}
}}

\caption{Comparison with SOTA methods under "inductive" GZS3 setting on VOC 2012 and COCO-Stuff 164k datasets.}
     \label{tab:compare-sota}
\vspace{-0.5em}
\end{table*}

% visualization
\begin{figure*}[!t]
\centering
        \includegraphics[width=0.98\textwidth]{cvpr_imgs/visualization.pdf}
\vspace{-0.3em}
\caption{\textbf{Visualization of segmentation prediction on COCO-Stuff 164k.} We compare the segmentation results between our approach and the SOTA method. The categories marked with \hl{red} are unseen classes and others are seen classes.}
\vspace{-1em}
\label{fig:visual}
\end{figure*}

\subsection{Setting}
\noindent\textbf{Datasets.} We evaluate our proposed method on two widely used datasets: VOC2012~\cite{everingham2011pascal} and COCO-Stuff 164K~\cite{caesar2018cvpr}. VOC2012 contains 10,582 augmented images for training and 1,449 for validation. Following previous works~\cite{zhou2022zegclip,ding2022decoupling}, we delete "background" class and use 15 classes as seen classes and 5 classes as unseen classes. COCO-Stuff 164K includes all 164K images from COCO~\cite{lin2014microsoft}, has 171 named categories and contains 118K images for training, 5K for evaluation. We use 156 classes as seen classes and 15 classes as unseen classes. The unseen classes of each dataset are shown in supplementary. 

\noindent\textbf{Metrics.} Following previous methods, we use three metrics to evaluate our results: mIoU(S), mIoU(U) and hIoU. mIoU(S) and mIoU(U) represent the mean Intersection over Union (mIoU) on seen classes and unseen classes, respectively. hIoU denotes the harmonic mean value of mIoU on seen and unseen classes: 
\[
hIoU = \frac{2\times mIoU(S)\times mIoU(U)}{mIoU(S)+mIoU(U)}.
\]

% need to modify 
\noindent\textbf{Implementation Details.} We implement our method based on the MMSegmentation~\cite{mmseg2020} framework. We choose CLIP ViT-B as our default vision and language backbones. The number of visual deep prompt tokens is set as 100 and 40 in each layer of CLIP for COCO-stuff 164k and VOC2012. The number of language deep prompt tokens is 6 in each layer on both datasets.
The number of our decoder block is 2. 
For local consensus self-attention, window size $n$ is 4$\times$4 total number of windows is 64 and the number of selected windows $m$ is 16. Following ZegCLIP, we linearly combine focal loss~\cite{lin2017focal} and dice loss~\cite{sudre2017generalised} as our training loss. The loss weights for focal loss and dice loss are 100.0 and 1.0, respectively. We crop each image into 512$\times$512 in both the training and evaluation stage. During training, we adopt AdamW~\cite{loshchilov2017decoupled} as our optimizer and set the initial learning rate as 2e-4. We use the polynomial learning rate scheduler. The number of iterations for COCO-Stuff 164k and VOC2012 is set as 80k and 20k, respectively. All experiments are conducted on 4 RTX3090 GPUs with the batch size of 16.





\subsection{Comparison with State-of-the-Arts}

To demonstrate the effectiveness of our method, we compare with previous the-state-of-art methods in Tab. \ref{tab:compare-sota} and also provide visualization results on the COCO-Stuff 164k dataset in Fig. \ref{fig:visual}. Both of them show the great generalization ability on unseen classes of our method.

\noindent\textbf{Inductive Settings.} First, we evaluate our method under inductive settings where the unseen class names are not known during training stage. From Tab. \ref{tab:compare-sota}, our method surpasses previous approaches on both VOC 2012 and COCO-Stuff 164k datasets. It outperforms DeOP~\cite{han2023zero} by 7.7\% and 6.4\% in mIoU(U) and hIoU on VOC 2012, and by 6.6\% and 5.9\% on COCO-Stuff 164k, respectively. Furthermore, our method exceeds the leading one-stage method ZegCLIP~\cite{zhou2022zegclip} by 4.5\% and 2.9\% in mIoU(U) and hIoU on VOC 2012, and by 3.6\% and 3.3\% on COCO-Stuff 164k.

\noindent\textbf{Visualization Results.} From Fig.~\ref{fig:visual}, we visualize some segmentation results from our method and the SOTA method on COCO-Stuff 164k validation dataset which contains more objects in a scene. The categories marked with red are unseen classes. From Fig.~\ref{fig:visual}, we can see that comparing with ZegCLIP, our method recognizes objects in the images more accurately and achieves a higher match with the ground truth classes. In addition, our method is more accurate in predicting unseen class masks, for example, as the red circled part in the bottom row of Fig.~\ref{fig:visual} shown, our method successfully distinguishes between "road" and "pavement", while ZegCLIP regards "pavement" as "road". And on the top of Fig.~\ref{fig:visual}, it illustrates that ZegCLIP segments the whole upper region of the image as the "clouds" category, while our method produces more fine-grained results that successfully distinguish between "clouds" and "sky-other", which is even more accurate than the ground truth annotation. 

\noindent\textbf{Trasductive Settings.} We also evaluate our method under transductive settings where the unseen class names are known during training stage. Thus, besides fine-tuning, this setting involves another self-tuning (ST) stage. We follows the same training strategy previous method~\cite{xu2022simple,zhou2022zegclip,kim2023zegot}. From Tab.~\ref{tab:transductive settings}, we compare our method with ZegOT and ZegCLIP on COCO-Stuff 164k datasets. Our method outperforms ZegOT by 2.9\% and 1.1\% on mIoU(S) and mIoU(U), respectively. Moreover our method exceeds ZegCLIP by 0.5\% and 0.4\% on mIoU(S) and mIoU(U), respectively. The results demonstrate that our method also performs well under transductive settings.

\noindent\textbf{Fully supervised.} We also provide the results of fully supervised semantic segmentation on COCO-Stuff 164k, which serves as the upper bound of our approach. In Tab.~\ref{tab:finetune-settings}, compared to ZegClip with 14M learnable parameters and ZegOT with 21M learnable parameters, our model has fewer parameters, specifically 11M. With less learnable parameters, our model still outperforms ZegOT and ZegCLIP by 5.3\% and 3.7\% on mIoU, respectively. These results demonstrate that our approach can better enhance the segmentation ability of CLIP’s backbone with less learnable parameters.
% transductive settings
\begin{table}[!t]
\centering
% \resizebox{0.8\linewidth}{!}{%
\setlength{\tabcolsep}{0.7em}
    {\renewcommand{\arraystretch}{1.1}
\begin{tabular}{cc|cl|cccc|cccc}
\toprule

\multicolumn{1}{c|}{Method} &\multicolumn{1}{c|}{mIoU(S)} & \multicolumn{1}{c|}{\textbf{mIoU(U)}}  & \multicolumn{1}{c}{hIoU} \\ \hline

\multicolumn{1}{c|}{ZegOT~\cite{kim2023zegot}+ST} & \multicolumn{1}{c|}{38.2} & \multicolumn{1}{c|}{59.2}    & \multicolumn{1}{c}{46.4} \\

\multicolumn{1}{c|}{ZegCLIP~\cite{zhou2022zegclip}+ST} & \multicolumn{1}{c|}{40.6} & \multicolumn{1}{c|}{59.9}    & \multicolumn{1}{c}{48.4} \\

\multicolumn{1}{c|}{Ours+ST} &\multicolumn{1}{c|}{\textbf{41.1}} & \multicolumn{1}{c|}{\textbf{60.3}}    & \multicolumn{1}{c}{\textbf{48.8}} \\

\bottomrule
\end{tabular}
}
% }
\caption{Comparison with SOTA methods under transductive ZS3 setting on COCO Stuff164k dataset. ``ST'' represents self-training.}
     \label{tab:transductive settings}

\end{table}

% table of full-fine tuning
\begin{table}[!t]
\centering
\resizebox{0.99\linewidth}{!}{%
\setlength{\tabcolsep}{0.7em}
    {\renewcommand{\arraystretch}{1.1}
\begin{tabular}{cc|cl|cccc|cccc}
\toprule

\multicolumn{1}{c|}{Method} &\multicolumn{1}{c|}{Params
}&\multicolumn{1}{c|}{mIoU} &\multicolumn{1}{c|}{mIoU(S)} & \multicolumn{1}{c|}{\textbf{mIoU(U)}}  & \multicolumn{1}{c}{hIoU} \\ \hline

\multicolumn{1}{c|}{ZegOT~\cite{kim2023zegot}} & \multicolumn{1}{c|}{21M} &\multicolumn{1}{c|}{40.1} &\multicolumn{1}{c|}{38.3} & \multicolumn{1}{c|}{58.7}    & \multicolumn{1}{c}{46.4} \\

\multicolumn{1}{c|}{ZegCLIP~\cite{zhou2022zegclip}} & \multicolumn{1}{c|}{14M} &\multicolumn{1}{c|}{42.7}&\multicolumn{1}{c|}{40.7} & \multicolumn{1}{c|}{63.2}    & \multicolumn{1}{c}{49.6} \\

\multicolumn{1}{c|}{Ours} & \multicolumn{1}{c|}{11M} & \multicolumn{1}{c|}{\textbf{46.4}}&\multicolumn{1}{c|}{\textbf{44.5}} & \multicolumn{1}{c|}{\textbf{65.9}}    & \multicolumn{1}{c}{\textbf{53.1}} \\

\bottomrule
\end{tabular}
}}
\caption{Comparison with SOTA methods under fully supervised semantic segmentation on COCO-Stuff 164k dataset, which serves as the upper bound of ZS3 methods.}
     \label{tab:finetune-settings}
\vspace{-0.3em}
\end{table}

\subsection{Ablation Study}

The effectiveness of LCTD decoder, the local consensus self-attention, and vision-language prompting is introduced for ablation studies. Besides, we compare the results with the different number of stacked decoder blocks, different initialization of the language prompt tuning, different length of language prompt tokens and different number of selected windows in local consensus self-attention. All ablation experiments are conducted on COCO-Stuff 164k validation dataset.

\begin{figure}[!t]
\centering
        \includegraphics[width=0.99\linewidth]{cvpr_imgs/decoder_align.pdf}
\vspace{-1em}
\caption{Visualization of cross attention between image features and class embeddings in our decoder with LCSA or without LCSA.}
\vspace{-1em}
\label{fig:intermediate cross attention map}
\end{figure}
% main ablation table
\begin{table}[!h]
\centering
\resizebox{1.0\linewidth}{!}{%
\setlength{\tabcolsep}{0.7em}
    {\renewcommand{\arraystretch}{1.1}
\begin{tabular}{cc|cl|cccc|cccc}
\toprule

\multicolumn{1}{c|}{Tuning Method} & \multicolumn{1}{c|}{Decoder} & \multicolumn{1}{c|}{mIoU(S)} & \multicolumn{1}{c|}{\textbf{mIoU(U)}}  & \multicolumn{1}{c}{hIoU} \\ \hline


\multicolumn{1}{c|}{Frozen} & \multicolumn{1}{c|}{SegViT} & \multicolumn{1}{c|}{32.3} & \multicolumn{1}{c|}{32.5}  & \multicolumn{1}{c}{32.4} \\
\rowcolor{gray!20}
\multicolumn{1}{c|}{Frozen} & \multicolumn{1}{c|}{LCTD(w/o LCSA)} & \multicolumn{1}{c|}{39.8} & \multicolumn{1}{c|}{41.1}  & \multicolumn{1}{c}{40.4} \\ \hline

\multicolumn{1}{c|}{VPT} & \multicolumn{1}{c|}{SegViT} & \multicolumn{1}{c|}{40.2} & \multicolumn{1}{c|}{41.4}  & \multicolumn{1}{c}{40.8} \\


\rowcolor{gray!20}
\multicolumn{1}{c|}{VPT} & \multicolumn{1}{c|}{LCTD(w/o LCSA)} & \multicolumn{1}{c|}{42.38} & \multicolumn{1}{c|}{43.82}  & \multicolumn{1}{c}{43.08} \\ \hline

\multicolumn{1}{c|}{VLPT} & \multicolumn{1}{c|}{LCTD(w/o LCSA)} & \multicolumn{1}{c|}{42.82} & \multicolumn{1}{c|}{44.22}  & \multicolumn{1}{c}{43.50} \\
\multicolumn{1}{c|}{VLPT} & \multicolumn{1}{c|}{SegViT} & \multicolumn{1}{c|}{42.3} & \multicolumn{1}{c|}{41.9}  & \multicolumn{1}{c}{42.2} \\
\rowcolor{gray!20}
\multicolumn{1}{c|}{VLPT} & \multicolumn{1}{c|}{LCTD} & \multicolumn{1}{c|}{\textbf{43.20}} & \multicolumn{1}{c|}{\textbf{45.02}}  & \multicolumn{1}{c}{\textbf{44.09}} \\
\bottomrule
\end{tabular}
}}
\caption{Comparison with different decoders in ZS3 under parameter free/efficient tuning.}
     \label{tab:main ablataion}
\vspace{-0.5em}
\end{table}

% number of selected windows
\begin{table}[!t]
\centering
% \resizebox{0.65\linewidth}{!}{%
\setlength{\tabcolsep}{0.7em}
    {\renewcommand{\arraystretch}{1.1}
\begin{tabular}{cc|cl|cccc|cccc}
\toprule

\multicolumn{1}{c|}{TopK} & \multicolumn{1}{c|}{mIoU(S)} & \multicolumn{1}{c|}{\textbf{mIoU(U)}}  & \multicolumn{1}{c}{hIoU} \\ \hline
\multicolumn{1}{c|}{8} & \multicolumn{1}{c|}{43.14} & \multicolumn{1}{c|}{44.87}    & \multicolumn{1}{c}{43.99} \\
\rowcolor{gray!20}
\multicolumn{1}{c|}{16} & \multicolumn{1}{c|}{43.20} & \multicolumn{1}{c|}{45.02}    & \multicolumn{1}{c}{44.09} \\
\multicolumn{1}{c|}{32} & \multicolumn{1}{c|}{43.20} & \multicolumn{1}{c|}{45.00}    & \multicolumn{1}{c}{44.08} \\

\multicolumn{1}{c|}{48} & \multicolumn{1}{c|}{42.98} & \multicolumn{1}{c|}{44.34}    & \multicolumn{1}{c}{43.64} \\

\bottomrule
\end{tabular}
}
% }
\vspace{-0.8em}
\caption{Ablation of the number of selected window in local consensus self-attention.}
     \label{tab:number of selected windows}
\vspace{-0.8em}
\end{table}

% number of decoder blocks

\begin{table}[!t]
\centering
% \resizebox{0.8\linewidth}{!}{%
\setlength{\tabcolsep}{0.7em}
    {\renewcommand{\arraystretch}{1.1}
\begin{tabular}{cc|cl|cccc|cccc}
\toprule

\multicolumn{1}{c|}{Number of Blocks} & \multicolumn{1}{c|}{mIoU(S)} & \multicolumn{1}{c|}{\textbf{mIoU(U)}}  & \multicolumn{1}{c}{hIoU} \\ \hline
\rowcolor{gray!20}
\multicolumn{1}{c|}{2} & \multicolumn{1}{c|}{43.20} & \multicolumn{1}{c|}{\textbf{45.02}}    & \multicolumn{1}{c}{\textbf{44.09}} \\
\multicolumn{1}{c|}{3} & \multicolumn{1}{c|}{43.06} & \multicolumn{1}{c|}{44.67}    & \multicolumn{1}{c}{43.85} \\
\multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{\textbf{44.01}} & \multicolumn{1}{c|}{43.26}    & \multicolumn{1}{c}{43.63} \\

\bottomrule
\end{tabular}
}
% }
\vspace{-0.8em}
\caption{Ablation of the number of decoder
blocks.}
     \label{tab:number of decoder blocks}
\vspace{-0.8em}
\end{table}

% \noindent\textbf{Switching QKV.} 
\noindent\textbf{Effectiveness of VLPT and LCTD.} 
One main difference between our LCTD decoder and SegViT decoder in ZegCLIP lies in that we choose image features as query and image features as key and value in cross attention of transformer decoder. As we illustrated in Sec.~\ref{introduce:explain}, under the parameter-free tuning and visual prompt tuning, the updating of visual space is limited, leading to a less structured visual space. This will increase the difficulty of alignment, thereby affecting the segmentation results. The results in Tab.~\ref{tab:main ablataion} demonstrate this point. Under parameter-free tuning, Our decoder with vanilla self-attention outperforms segvit decoder by 7.5\% and 8.6\% on mIoU(S) and mIoU(U), respectively. Under visual prompt tuning, our decoder decoder with vanilla self-attention also gains by 2.1\% and 2.4\%, respectively. These highlight the necessity of explicitly updating the visual space in one-stage method.

\noindent\textbf{Local Consensus Self-Attention.} In our local consensus transformer decoder, we replace vanilla self-attention with local consensus self attention to enhance the local semantic consensus in the same object. In Tab.~\ref{tab:main ablataion}, after introducing local consensus self-attention, the mIoU(S) and mIoU(U) increase by 0.38\% and 0.8\%, respectively. In Fig.~\ref{fig:intermediate cross attention map}, we visualize the cross attention map in the last block of our decoder. We observe that after incorporating local consensus self-attention, the noise in the cross-attention map is reduced, and the semantics within the same object become more consistent, which demonstrate the effectiveness of local consensus self-attention. Besides, we give the ablation study about the number of selected windows in local consensus self-attention in Tab.~\ref{tab:number of selected windows}. The total number of windows in patch features is 64. In Tab.~\ref{tab:number of selected windows}, the results show the constant performance when the number is 16 and 32. However, when the number is 48, the local consensus self-attention starts behaving like vanilla self-attention, gathering too many irrelevant patches, leading to a performance decline.

\noindent\textbf{Number of Decoder Blocks.} In Tab.~\ref{tab:number of decoder blocks}, we evaluate the impact of the number of decoder blocks on ZS3 performance. A lightweight local consensus transformer decoder with two block is already sufficient.
% ly competent for this task. 
% There is almost no difference in 
The performances are similar between a two-layer decoder and a three-layer decoder. Increasing the number of layers leads to a decrease in mIoU(U). Considering both the number of parameters and performance, we stack two decoder blocks. This choice also results in our approach having fewer learnable parameters compared to ZegCLIP, with a total of 11M learnable parameters.



\noindent\textbf{Vision Language Prompt Tuning.}
We compare different prompt tuning methods, as shown in Tab.~\ref{tab:prompt methods}. It illustrates that applying deep prompt tuning on both vision and language backbone simultaneously brings the best performance on both seen and unseen classes. If deep prompt tuning is only applied to the language backbone, the performance will decrease 2.28\% and 5.54\% on seen and unseen classes, respectively. If deep prompt tuning is only applied to the vision backbone, the performance will decrease 0.94\% and 1.92\%, respectively. The results also show that prompt tuning on the vision backbone has more effects on segmentation performance. 




\noindent\textbf{Initialization of Language Prompt.} In Tab.~\ref{tab:prompt initialize}, we compare different prompt initialization methods on the language backbone. ``Random'' means we use random Gaussian distribution to initialize prompts and ``pretrain'' means we use the initial strategy mentioned in Sec~\ref{par:VLPT}. From the results, the proposed "pretrain" initialization is better than random initialization, especially prominent in unseen classes, where it achieves 4.5\% mIoU gain compared to the random initialization. Besides, in Tab.~\ref{tab:prompt len}, we show the impact of length of initialized language prompts. The results indicates that more language prompt tokens leads to a better performance on segmentation about unseen classes.

% vision language prompt tuning
\begin{table}[!t]
\centering
% \resizebox{0.8\linewidth}{!}{%
\setlength{\tabcolsep}{0.7em}
    {\renewcommand{\arraystretch}{1.1}
\begin{tabular}{cc|cl|cccc|cccc}
\toprule

\multicolumn{1}{c|}{Prompt Tuning} & \multicolumn{1}{c|}{mIoU(S)} & \multicolumn{1}{c|}{\textbf{mIoU(U)}}  & \multicolumn{1}{c}{hIoU} \\ \hline
\multicolumn{1}{c|}{Language-Only} & \multicolumn{1}{c|}{40.92} & \multicolumn{1}{c|}{39.48}    & \multicolumn{1}{c}{40.19} \\
\multicolumn{1}{c|}{Vision-Only} & \multicolumn{1}{c|}{42.26} & \multicolumn{1}{c|}{43.10}    & \multicolumn{1}{c}{42.68} \\
\rowcolor{gray!20}
\multicolumn{1}{c|}{Vision-Language} & \multicolumn{1}{c|}{\textbf{43.20}} & \multicolumn{1}{c|}{\textbf{45.02}}    & \multicolumn{1}{c}{\textbf{44.09}} \\


\bottomrule
\end{tabular}
}
% }
% \vspace{-0.5em}
\caption{Ablation of different prompt tuning on CLIP's encoders.}
     \label{tab:prompt methods}
% \vspace{-1.4em}
\end{table}

% language prompt initialization approach

\begin{table}[!t]
\centering
% \resizebox{0.8\linewidth}{!}{%
\setlength{\tabcolsep}{0.7em}
    {\renewcommand{\arraystretch}{1.1}
\begin{tabular}{cc|cl|cccc|cccc}
\toprule

\multicolumn{1}{c|}{Prompt Init.}  & \multicolumn{1}{c|}{mIoU(S)} & \multicolumn{1}{c|}{\textbf{mIoU(U)}}  & \multicolumn{1}{c}{hIoU} \\ \hline

\multicolumn{1}{c|}{Random}  & \multicolumn{1}{c|}{43.13} & \multicolumn{1}{c|}{40.5}  & \multicolumn{1}{c}{41.77} \\
\rowcolor{gray!20}
\multicolumn{1}{c|}{Pretrain}  & \multicolumn{1}{c|}{\textbf{43.2}} & \multicolumn{1}{c|}{\textbf{45.02}}  & \multicolumn{1}{c}{\textbf{44.09}} \\


\bottomrule
\end{tabular}
}
% }
\caption{Ablation of different language prompt initialization
strategies.}
     \label{tab:prompt initialize}

\end{table}

% language prompt length approach
\begin{table}[!t]
\centering
\resizebox{0.99\linewidth}{!}{%
\setlength{\tabcolsep}{0.7em}
    {\renewcommand{\arraystretch}{1.1}
\begin{tabular}{cc|cl|cccc|cccc}
\toprule

\multicolumn{1}{c|}{Length} & \multicolumn{1}{c|}{Initialized Template} & \multicolumn{1}{c|}{mIoU(S)} & \multicolumn{1}{c|}{\textbf{mIoU(U)}}  & \multicolumn{1}{c}{hIoU} \\ \hline
\multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{"a photo of a"} & \multicolumn{1}{c|}{\textbf{43.26}} & \multicolumn{1}{c|}{43.4}    & \multicolumn{1}{c}{43.33} \\
\multicolumn{1}{c|}{5} & \multicolumn{1}{c|}{"a cropped photo of the"} & \multicolumn{1}{c|}{43.07} & \multicolumn{1}{c|}{43.97}    & \multicolumn{1}{c}{43.52} \\
\rowcolor{gray!20}
\multicolumn{1}{c|}{6} & \multicolumn{1}{c|}{"This is a photo of a"} & \multicolumn{1}{c|}{43.20} & \multicolumn{1}{c|}{\textbf{45.02}}    & \multicolumn{1}{c}{\textbf{44.09}} \\
\bottomrule
\end{tabular}
}
}
\caption{Analysis of the impact of the length of language prompt tokens.}
     \label{tab:prompt len}

\end{table}


==> sec/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
\textcolor{red}{Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sections/Abstract.tex <==
\begin{abstract}
Vision-language pre-trained model, $e.g.$, Contrastive Language-Image Pretraining (CLIP), facilitates zero-shot semantic segmentation by aligning visual features with language embeddings through cross-attention.
%
The existing cross-attention mechanism, despite of simplicity, ignores that the embedding of class names is sparse and distinct within the semantic space.
%
For the sparse and distinct text embedding, is it possible to aggregate the visual features to separable subspaces to increase discrimination capacity?
%
%However, the semantic typology of text embedding is rarely considered, which is distinct and stable in the semantic space.
%红色的这句意思不对
In this paper, we propose a \textbf{S}emantic \textbf{C}ompressed \textbf{V}isual \textbf{R}epresentation (SCVR) approach for zero-shot semantic segmentation, where visual features are forced to be close to the embedding of class names.  
%
Specifically, we use visual features as the query for cross-attention in contrast to the existing ones using language embedding.
%
In this simple-yet-effective way, the visual features of the same category are updated thoroughly to approach the unique semantic center.
%
Equipped with a visual-language prompting strategy, SCVR significantly improves the generalization capacity of segmentation models on unseen classes.
%
Experiments show that SCVR achieves mIoU gains of unseen classes with 4.5\% on the PASCAL VOC 2012 and 3.6\% on the COCO-Stuff 164k compared with the state-of-the-art, respectively.
\end{abstract}

==> sections/Conclusion.tex <==
\section{Conclusion}
We propose a  Semantic Compressed Visual Representation for zero-shot semantic segmentation, in which we make SCVR decoder iteratively update visual features to increase the similarity with the text embeddings of class categories. The semantic compression is achieved through a simple transformer-based decoder, using visual features as query and class name embeddings as key and value. Besides, under a visual-language prompting strategy, SCVR further improves segmentation capabilities on unseen classes. Extensive experiments have demonstrated the effectiveness of our method. Due to the reliance of our method on the guidance of the class name embeddings and the existing datasets often suffer from ambiguous object label annotations, such as "wall-other" and "sky-other" in COCO, it leads to misclassification with the proposed SCVR.
% We hope the community can work together to improve this issue.  


==> sections/Experiment.tex <==
\section{Experiment}


\subsection{Setting}
\noindent\textbf{Datasets.} We evaluate our proposed method on two widely used datasets: VOC2012~\cite{everingham2011pascal} and COCO-Stuff 164K~\cite{caesar2018cvpr}. VOC2012 contains 10,582 augmented images for training and 1,449 for validation. Following previous works~\cite{zhou2022zegclip,ding2022decoupling}, we delete "background" class and use 15 classes as seen classes and 5 classes as unseen classes. COCO-Stuff 164K includes all 164K images from COCO~\cite{lin2014microsoft}, has 171 named categories and contains 118K images for training, 5K for evaluation. We use 156 classes as seen classes and 15 classes as unseen classes. The unseen classes of each dataset are shown in supplementary. 

\noindent\textbf{Metrics.} Following previous methods, we use three metrics to evaluate our results: mIoU(S), mIoU(U) and hIoU. mIoU(S) and mIoU(U) represent the mean Intersection over Union (mIoU) on seen classes and unseen classes, respectively. hIoU denotes the harmonic mean value of mIoU on seen and unseen classes: 
\[
hIoU = \frac{2\times mIoU(S)\times mIoU(U)}{mIoU(S)+mIoU(U)}.
\]

% need to modify 
\noindent\textbf{Implementation Details.} We implement our method based on the mmsegmentation~\cite{mmseg2020} framework. We choose CLIP ViT-B as our default vision and language backbones. The number of visual deep prompt tokens is set as 100 and 40 in each layer of CLIP for COCO-stuff 164k and VOC2012. The number of language deep prompt tokens is 6 in each layer on both datasets.
The number of our decoder block is 2. 
For local self-attention, window size $n$ is 4$\times$4 and $m$ is 16. Following ZegCLIP, we linearly combine focal loss~\cite{lin2017focal} and dice loss~\cite{sudre2017generalised} as our training loss. The loss weights for focal loss and dice loss are 100.0 and 1.0, respectively. We crop each image into 512$\times$512 in both the training and evaluation stage. During training, we adopt AdamW~\cite{loshchilov2017decoupled} as our optimizer and set the initial learning rate as 2e-4. We use the polynomial learning rate scheduler. The number of iterations for COCO-Stuff 164k and VOC2012 is set as 80k and 20k, respectively. All experiments are conducted on 4 RTX3090 GPUs with the batch size of 16.


\subsection{Comparison with State-of-the-Arts}

To demonstrate the effectiveness of our method, we compare with previous the-state-of-art methods in Tab. \ref{tab:compare-sota} and also provide visualization results on the COCO-Stuff 164k dataset in Fig. \ref{fig:visual}. Both of them show the great generalization ability on unseen classes of our method.

\noindent\textbf{Numerical results.} From Tab. \ref{tab:compare-sota}, our method surpasses previous approaches on both VOC 2012 and COCO-Stuff 164k datasets. It outperforms the state-of-the-art two-stage method DeOP~\cite{han2023zero} by 7.7\% and 6.4\% in mIoU(U) and hIoU on VOC 2012, and by 6.6\% and 5.9\% on COCO-Stuff 164k, respectively. Moreover, our method exceeds the leading one-stage method ZegCLIP~\cite{zhou2022zegclip} by 4.5\% and 2.9\% in mIoU(U) and hIoU on VOC 2012, and by 3.6\% and 3.3\% on COCO-Stuff 164k.

\noindent\textbf{Visualization results.} From Fig.~\ref{fig:visual}, we visualize some segmentation results from our method and the SOTA method on COCO-Stuff 164k validation dataset which contains more objects in a scene. The categories marked with red are unseen classes. From Fig.~\ref{fig:visual}, we can see that comparing with ZegCLIP, our method recognizes objects in the images more accurately and achieves a higher match with the ground truth classes. In addition, our method is more accurate in predicting unseen class masks, for example, as the red circled part in the bottom row of Fig.~\ref{fig:visual} shown, our method successfully distinguishes between "road" and "pavement", while ZegCLIP regards "pavement" as "road". And on the top of Fig.~\ref{fig:visual}, it illustrates that ZegCLIP segments the whole upper region of the image as the "clouds" category, while our method produces more fine-grained results that successfully distinguish between "clouds" and "sky-other". 

\begin{table}[]
\centering
\resizebox{0.99\linewidth}{!}{%
\setlength{\tabcolsep}{0.7em}
    {\renewcommand{\arraystretch}{1.1}
\begin{tabular}{cc|cl|cccc|cccc}
\toprule
\multicolumn{2}{l|}{} &\multicolumn{1}{l|}{\multirow{2}{*}{Type}} &\multicolumn{1}{l|}{\multirow{2}{*}{Pipeline}}      & \multicolumn{4}{c|}{\textbf{PASCAL VOC 2012}} &\multicolumn{4}{c}{\textbf{COCO-Stuff 164k}}
\\ \cline{5-12} 

\multicolumn{2}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{pAcc}            & \multicolumn{1}{c|}{mIoU(S)}          & \multicolumn{1}{c|}{\textbf{mIoU(U)}} &\multicolumn{1}{c|}{hIoU}& \multicolumn{1}{c|}{pAcc}            & \multicolumn{1}{c|}{mIoU(S)}          & \multicolumn{1}{c|}{\textbf{mIoU(U)}} &\multicolumn{1}{c}{hIoU}\\ \hline

\multicolumn{2}{l|}{SPNet~\cite{xian2019semantic}} &\multicolumn{1}{l|}{Discriminative} & \multicolumn{1}{l|}{One-Stage}     & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ 78.0 } & \multicolumn{1}{c|}{ 15.6 } & \multicolumn{1}{c|}{ 26.1 } & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ 35.2 } & \multicolumn{1}{c|}{ 8.7 } & \multicolumn{1}{c}{ 14.0 }         \\

\multicolumn{2}{l|}{ZS3~\cite{bucher2019zero}} &\multicolumn{1}{l|}{Generative} & \multicolumn{1}{l|}{One-Stage}     & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ 77.3 } & \multicolumn{1}{c|}{ 17.7 } & \multicolumn{1}{c|}{ 28.7 } & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ 34.7 } & \multicolumn{1}{c|}{ 9.5 } & \multicolumn{1}{c}{ 15.0 }         \\ 

\multicolumn{2}{l|}{CaGNet~\cite{gu2020context}} &\multicolumn{1}{l|}{Generative} & \multicolumn{1}{l|}{One-Stage}     & \multicolumn{1}{c|}{ 80.7 } & \multicolumn{1}{c|}{ 78.4 } & \multicolumn{1}{c|}{ 26.6 } & \multicolumn{1}{c|}{ 39.7 } & \multicolumn{1}{c|}{ 56.6 } & \multicolumn{1}{c|}{ 33.5 } & \multicolumn{1}{c|}{ 12.2 } & \multicolumn{1}{c}{ 18.2 }         \\ 

\multicolumn{2}{l|}{SIGN~\cite{cheng2021sign}} &\multicolumn{1}{l|}{Generative} & \multicolumn{1}{l|}{One-Stage}     & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ 75.4 } & \multicolumn{1}{c|}{ 28.9 } & \multicolumn{1}{c|}{ 41.7 } & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ 32.3 } & \multicolumn{1}{c|}{ 15.5 } & \multicolumn{1}{c}{ 20.9 }         \\ 
\multicolumn{2}{l|}{Joint~\cite{baek2021exploiting}} &\multicolumn{1}{l|}{Discriminative} & \multicolumn{1}{l|}{One-Stage}     & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ 77.7 } & \multicolumn{1}{c|}{ 32.5 } & \multicolumn{1}{c|}{ 45.9 } & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c}{ - }         \\

\multicolumn{2}{l|}{STRICT~\cite{pastore2021closer}} &\multicolumn{1}{l|}{Discriminative} & \multicolumn{1}{l|}{One-Stage}     & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ 82.7 } & \multicolumn{1}{c|}{ 35.6 } & \multicolumn{1}{c|}{ 49.8 } & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ 35.3 } & \multicolumn{1}{c|}{ 30.3 } & \multicolumn{1}{c}{ 32.6 }         \\

\multicolumn{2}{l|}{ZegFormer~\cite{ding2022decoupling}} &\multicolumn{1}{l|}{Discriminative} & \multicolumn{1}{l|}{Two-Stage}     & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ 86.4 } & \multicolumn{1}{c|}{ 63.6 } & \multicolumn{1}{c|}{ 73.3 } & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ 36.6 } & \multicolumn{1}{c|}{ 33.2 } & \multicolumn{1}{c}{ 34.8 }         \\

\multicolumn{2}{l|}{Zsseg~\cite{xu2022simple}} &\multicolumn{1}{l|}{Discriminative} & \multicolumn{1}{l|}{Two-Stage}     & \multicolumn{1}{c|}{ 90.0 } & \multicolumn{1}{c|}{ 83.5 } & \multicolumn{1}{c|}{ 72.5 } & \multicolumn{1}{c|}{ 77.5 } & \multicolumn{1}{c|}{ 60.3 } & \multicolumn{1}{c|}{ 39.3 } & \multicolumn{1}{c|}{ 36.3 } & \multicolumn{1}{c}{ 37.8 }         \\

\multicolumn{2}{l|}{DeOP~\cite{han2023zero}} &\multicolumn{1}{l|}{Discriminative} & \multicolumn{1}{l|}{Two-Stage}     & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ 88.2 } & \multicolumn{1}{c|}{ 74.6 } & \multicolumn{1}{c|}{ 80.8 } & \multicolumn{1}{c|}{ - } & \multicolumn{1}{c|}{ 38.0 } & \multicolumn{1}{c|}{ 38.4 } & \multicolumn{1}{c}{ 38.2 }         \\

\multicolumn{2}{l|}{ZegCLIP~\cite{zhou2022zegclip}} &\multicolumn{1}{l|}{Discriminative} & \multicolumn{1}{l|}{One-Stage}     & \multicolumn{1}{c|}{ 94.6 } & \multicolumn{1}{c|}{ 91.9 } & \multicolumn{1}{c|}{ 77.8 } & \multicolumn{1}{c|}{ 84.3 } & \multicolumn{1}{c|}{ 62.0 } & \multicolumn{1}{c|}{ 40.2 } & \multicolumn{1}{c|}{ 41.4 } & \multicolumn{1}{c}{ 40.8 } \\ \hline

\multicolumn{2}{l|}{SCVR(Ours)} &\multicolumn{1}{l|}{Discriminative}  & \multicolumn{1}{l|}{One-Stage}     & \multicolumn{1}{c|}{ \textbf{95.5} } & \multicolumn{1}{c|}{ \textbf{92.5} } & \multicolumn{1}{c|}{ \textbf{82.3} } & \multicolumn{1}{c|}{ \textbf{87.2} } & \multicolumn{1}{c|}{ \textbf{64.3} } & \multicolumn{1}{c|}{ \textbf{43.2} } & \multicolumn{1}{c|}{ \textbf{45.0} } & \multicolumn{1}{c}{ \textbf{44.1} } \\ \bottomrule
\end{tabular}
}}
\vspace{0.5em}
\caption{Comparison with SOTA methods under "inductive" GZS3 setting on VOC 2012 and COCO-Stuff 164k datasets.}
     \label{tab:compare-sota}
\end{table}

% 调整表格之间的间距
\vspace{2em}

\begin{figure}[!t]
\centering
        \includegraphics[width=0.99\textwidth]{imgs/visual.pdf}
\vspace{-1em}
\caption{Visualization of segmentation prediction on COCO-Stuff 164k. The categories marked with red are unseen classes and others are seen classes.}
\label{fig:visual}
\end{figure}



\subsection{Ablation Study}

% \begin{figure}[t]
% \centering
%   \includegraphics[width=0.98\textwidth]{imgs/decoder_arch.pdf}
% \caption{Different types of decoder for semantic segmentation. (a) The integrated language-vision feature is used as the query and key with self-attention. (b) The language feature is used as the query and the visual feature is used as the key with cross-attention. (c) We use language features as the key to compress the visual space.}
% \label{fig:decoder}
% \end{figure}

The effectiveness of SCVR decoder, the local self-attention, and vision-language prompting is introduced for ablation studies. Besides, we compare the results with the different numbers of stacked decoder blocks and different initialization of the language prompt tuning.  
All experiments are conducted on COCO-Stuff 164k validation dataset.

\textbf{SCVR Decoder.} 
% We verify the effectiveness of SCVR decoder from two aspects: numerical results and visualization results. 
,In Tab.~\ref{tab:different decoders}, we compare different types of ZS3 decoders under parameter-free fine-tuning, full fine-tuning, and vision-language prompt tuning circumstances. We enumerate three types of decoders: a) segmenter decoder~\cite{strudel2021segmenter} which concatenates dense visual features with text features and leverages transformer encoder with self-attention, b) ZegCLIP~\cite{zhou2022zegclip} decoder which uses transformer decoder block to update text features with cross-attention, and c) our SCVR decoder which utilizes transformer decoder block to update dense visual features with cross-attention. As discussed in \ref{par:explicit update}, explicit updating visual space with the proposed decoder can compensate for the drawback of frozen tuning and prompt tuning. The results in Tab.~\ref{tab:different decoders} demonstrate this perspective. 
Under parameter-free fine-tuning circumstances in which visual space is not updated, 
% Comparing with ZegCLIP decoder, under parameter-free fine-tuning circumstances in which visual space can't be implicitly updated by gradients, 
our decoder outperforms ZegCLIP decoder by 7.5\% and 7.6\% on mIoU(S) and mIoU(U), respectively. Under visual-language prompt tuning, ZegCLIP decoder only implicitly updates the visual space to a limited extent through gradient propagation while our decoder explicitly updates the visual space. The proposed decoder outperforms ZegCLIP by 0.9\% and 3.1\%, respectively. 

We visualize the alignment maps between dense visual features and text features. which can be viewed as the spatial distribution of a certain category in the image. The alignment maps of the input and output with different decoders are shown in Fig.~\ref{fig:explain}.  
% before and after our decoder and ZegCLIP decoder.
% Due to implicit updating by gradient propagation, the features before the ZegCLIP decoder align better than our decoder, while the output features of our decoder align much better than ZegCLIP for explicit updating.
Due to explicit updating of visual space, the output features of our decoder align much better than ZegCLIP.

\begin{figure}[!t]
\centering
        \includegraphics[width=0.98\textwidth]{imgs/explain.pdf}
\vspace{-1em}
\caption{Visualizing the alignment maps between visual features and text features before and after our decoder and ZegCLIP decoder.}

\label{fig:explain}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  comparing different decoders under freeze, fine-tune, prompt tuning
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[!t]
\centering
\resizebox{0.99\linewidth}{!}{%
\setlength{\tabcolsep}{0.7em}
    {\renewcommand{\arraystretch}{1.1}
\begin{tabular}{cc|cl|cccc|cccc}
\toprule
\multicolumn{1}{l|}{\multirow{2}{*}{Different ZS3 decoders}} & \multicolumn{3}{c|}{Parameter-free Fine-tuning} &\multicolumn{3}{c|}{Full Fine-tuning} & \multicolumn{3}{c}{VL Prompt Tuning}
\\ \cline{2-10} 

\multicolumn{1}{l|}{}    & \multicolumn{1}{c|}{mIoU(S)}          & \multicolumn{1}{c|}{\textbf{mIoU(U)}} &\multicolumn{1}{c|}{hIoU}  & \multicolumn{1}{c|}{mIoU(S)}          & \multicolumn{1}{c|}{\textbf{mIoU(U)}} &\multicolumn{1}{c|}{hIoU}
& \multicolumn{1}{c|}{mIoU(S)}          & \multicolumn{1}{c|}{\textbf{mIoU(U)}} &\multicolumn{1}{c}{hIoU}
\\ \hline

\multicolumn{1}{l|}{Segmenter decoder~\cite{strudel2021segmenter}}    & \multicolumn{1}{c|}{37.4}          & \multicolumn{1}{c|}{34.7} &\multicolumn{1}{c|}{36.0}  & \multicolumn{1}{c|}{43.9}          & \multicolumn{1}{c|}{31.3} &\multicolumn{1}{c|}{36.6}
& \multicolumn{1}{c|}{41.1}          & \multicolumn{1}{c|}{40.4} &\multicolumn{1}{c}{40.8} \\ 
\multicolumn{1}{l|}{ZegCLIP decoder~\cite{zhou2022zegclip}}    & \multicolumn{1}{c|}{32.3}          & \multicolumn{1}{c|}{32.5} &\multicolumn{1}{c|}{32.4}  & \multicolumn{1}{c|}{42.7}          & \multicolumn{1}{c|}{22.3} &\multicolumn{1}{c|}{29.3}
& \multicolumn{1}{c|}{42.3}          & \multicolumn{1}{c|}{41.9} &\multicolumn{1}{c}{42.2} \\ 
\multicolumn{1}{l|}{Our decoder}    & \multicolumn{1}{c|}{\textbf{39.8}}          & \multicolumn{1}{c|}{\textbf{41.1}} &\multicolumn{1}{c|}{\textbf{40.4}}  & \multicolumn{1}{c|}{\textbf{44.1}}          & \multicolumn{1}{c|}{\textbf{35.7}} &\multicolumn{1}{c|}{\textbf{39.5}}
& \multicolumn{1}{c|}{\textbf{43.2}}          & \multicolumn{1}{c|}{\textbf{45.0}} &\multicolumn{1}{c}{\textbf{44.1}} \\ 
\bottomrule
\end{tabular}
}}
\vspace{0.2em}
\caption{Comparison with different ZS3 decoders under parameter-free/full fine-tuning and prompt tuning settings.}
     \label{tab:different decoders}
\vspace{-1em}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  decoder components ablation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[!t]
\begin{minipage}{.49\linewidth}
\centering
\resizebox{\linewidth}{!}{{
\setlength{\tabcolsep}{0.5em}
    {\renewcommand{\arraystretch}{1.0}
    \begin{tabular}{|c|c|c|c|c|}
\toprule

\multicolumn{1}{c|}{Types of self-attention} & \multicolumn{1}{c|}{mIoU(S)} & \multicolumn{1}{c|}{\textbf{mIoU(U)}}  & \multicolumn{1}{c}{hIoU} \\ \hline
\multicolumn{1}{c|}{Global attention} & \multicolumn{1}{c|}{42.38} & \multicolumn{1}{c|}{43.97}    & \multicolumn{1}{c}{43.16} \\
\multicolumn{1}{c|}{Local attention} & \multicolumn{1}{c|}{\textbf{43.20}} & \multicolumn{1}{c|}{\textbf{45.02}}    & \multicolumn{1}{c}{\textbf{44.09}} \\

 \bottomrule
 \end{tabular}
    }}}
\vspace{0.2em}
\caption{Ablation of different types of self-attention in decoder.}
\label{tab:attention types}
\end{minipage}
\hspace{0.02\linewidth}
\begin{minipage}{.49\linewidth}
\centering

\resizebox{\linewidth}{!}{{
\setlength{\tabcolsep}{0.5em}
    {\renewcommand{\arraystretch}{1.0}
    \begin{tabular}{|c|c|c|c|c|}
\toprule
% \multicolumn{1}{c|}{Number of layers} & \multicolumn{1}{c|}{mIoU(S)} & \multicolumn{1}{c|}{\textbf{mIoU(U)}}  & \multicolumn{1}{c}{hIoU} \\ \hline
% \multicolumn{1}{c|}{2} & \multicolumn{1}{c|}{43.20} & \multicolumn{1}{c|}{\textbf{45.02}}    & \multicolumn{1}{c}{\textbf{44.09}} \\
% \multicolumn{1}{c|}{3} & \multicolumn{1}{c|}{43.06} & \multicolumn{1}{c|}{44.67}    & \multicolumn{1}{c}{43.85} \\
% \multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{\textbf{44.01}} & \multicolumn{1}{c|}{43.26}    & \multicolumn{1}{c}{43.63} \\
\multicolumn{1}{c|}{Prompt Tuning} & \multicolumn{1}{c|}{mIoU(S)} & \multicolumn{1}{c|}{\textbf{mIoU(U)}}  & \multicolumn{1}{c}{hIoU} \\ \hline
\multicolumn{1}{c|}{Language-Only} & \multicolumn{1}{c|}{40.92} & \multicolumn{1}{c|}{39.48}    & \multicolumn{1}{c}{40.19} \\
\multicolumn{1}{c|}{Vision-Only} & \multicolumn{1}{c|}{42.26} & \multicolumn{1}{c|}{43.10}    & \multicolumn{1}{c}{42.68} \\
\multicolumn{1}{c|}{Vision-Language} & \multicolumn{1}{c|}{\textbf{43.20}} & \multicolumn{1}{c|}{\textbf{45.02}}    & \multicolumn{1}{c}{\textbf{44.09}} \\
 \bottomrule
 \end{tabular}}}
}
\vspace{0.1em}
\caption{Ablation of the number of decoder blocks.}
% \label{tab:decoder layers}
\label{tab:prompt methods}
\end{minipage}
\vspace{-2em}
\end{table}


\noindent\textbf{Local Self-Attention.} In our decoder, we replace global self-attention with local self-attention, which can better aggregate local context information to update visual features. In Tab.~\ref{tab:attention types}, when substituting global attention with local attention, mIoU(S) and mIoU(U) are increased by 0.82\% and 1.05\%. 

\noindent\textbf{Vision-Language Prompt Tuning.} We compare different prompt tuning methods, as shown in Tab.~\ref{tab:prompt methods}. It illustrates that applying deep prompt tuning on both vision and language backbone simultaneously brings the best performance on both seen and unseen classes. If deep prompt tuning is only applied to the language backbone, the performance will decrease 2.28\% and 5.54\% on seen and unseen classes, respectively. If deep prompt tuning is only applied to the vision backbone, the performance will decrease 0.94\% and 1.92\%, respectively. The results also show that prompt tuning on the vision backbone has more effects on segmentation performance. 

\noindent\textbf{Number of Decoder Blocks.} In Tab.~\ref{tab:decoder layers}, we evaluate the impact of the number of decoder blocks on ZS3 performance. A lightweight SCVR decoder with two layers is already sufficient.
% ly competent for this task. 
% There is almost no difference in 
The performances are similar between a two-layer decoder and a three-layer decoder. Increasing the number of layers leads to a decrease in mIoU(U). Considering both the number of parameters and performance, we stack two decoder blocks. 

In Fig.~\ref{fig:propagate}, we visualize alignment maps between visual features and text features at the encoder, 1st decoder block, and  2nd decoder block, respectively. The visualization shows that the decoder progressively updates the visual feature to converge toward the corresponding class embedding.

\noindent\textbf{Initialization for Language Prompt Tuning.}
In Tab.~\ref{tab:prompt initialization}, we compare different prompt initialization methods on the language backbone. "Shallow" represents inserting learnable prompts at the first layer like CoOP~\cite{zhou2022learning} and "Deep" inserting learnable prompts at each layer. "random" means we use random Gaussian distribution to initialize prompts and "pretrain" means we use the initial strategy mentioned in Sec.~\ref{par:initialization}. From the results, we can see that deep prompt tuning is better than shallow prompt tuning by 0.39\% and 2.62\%, respectively. And the proposed "pretrain" initialization is better than random initialization, especially prominent in unseen classes, where it achieves 4.5\% mIoU gain compared to the random initialization.

% \textbf{The Effectiveness of Class Weight Generator.} In Tab.~\ref{tab:decoder component}, we evaluate the effectiveness of the class weight generator. We find that with class-wise scaling, our model can increase mIoU(U) by 1.62\% comparing with without class-wise scaling, which demonstrates class-wise scaling can improve segmentation prediction on unseen classes.

\begin{figure}[!t]
\centering
        \includegraphics[width=0.98\textwidth]{imgs/propagate.pdf}
\vspace{-1em}
\caption{Visualization of aligned maps between visual features and text features through SCVR decoder. For each category, it shows the aligned maps of the outputs of the CLIP encoder, the 1st decoder block, and the 2nd decoder block, respectively.}
\label{fig:propagate}
\vspace{-0.5em}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  encoder part ablation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[!t]
\begin{minipage}{.44\linewidth}
\centering
\resizebox{\linewidth}{!}{{
\setlength{\tabcolsep}{0.5em}
    {\renewcommand{\arraystretch}{1.0}
    \begin{tabular}{|c|c|c|c|c|}
\toprule
% \multicolumn{1}{c|}{Prompt Tuning} & \multicolumn{1}{c|}{mIoU(S)} & \multicolumn{1}{c|}{\textbf{mIoU(U)}}  & \multicolumn{1}{c}{hIoU} \\ \hline
% \multicolumn{1}{c|}{Language-Only} & \multicolumn{1}{c|}{40.92} & \multicolumn{1}{c|}{39.48}    & \multicolumn{1}{c}{40.19} \\
% \multicolumn{1}{c|}{Vision-Only} & \multicolumn{1}{c|}{42.26} & \multicolumn{1}{c|}{43.10}    & \multicolumn{1}{c}{42.68} \\
% \multicolumn{1}{c|}{Vision-Language} & \multicolumn{1}{c|}{\textbf{43.20}} & \multicolumn{1}{c|}{\textbf{45.02}}    & \multicolumn{1}{c}{\textbf{44.09}} \\
\multicolumn{1}{c|}{Number of layers} & \multicolumn{1}{c|}{mIoU(S)} & \multicolumn{1}{c|}{\textbf{mIoU(U)}}  & \multicolumn{1}{c}{hIoU} \\ \hline
\multicolumn{1}{c|}{2} & \multicolumn{1}{c|}{43.20} & \multicolumn{1}{c|}{\textbf{45.02}}    & \multicolumn{1}{c}{\textbf{44.09}} \\
\multicolumn{1}{c|}{3} & \multicolumn{1}{c|}{43.06} & \multicolumn{1}{c|}{44.67}    & \multicolumn{1}{c}{43.85} \\
\multicolumn{1}{c|}{4} & \multicolumn{1}{c|}{\textbf{44.01}} & \multicolumn{1}{c|}{43.26}    & \multicolumn{1}{c}{43.63} \\
 \bottomrule
 \end{tabular}
    }}}
\vspace{0.2em}
\caption{Ablation of different prompt tuning methods.}
% \label{tab:prompt methods}
\label{tab:decoder layers}
\end{minipage}
\hspace{0.02\linewidth}
\begin{minipage}{0.54\linewidth}
\centering
\resizebox{\linewidth}{!}{{
\setlength{\tabcolsep}{0.5em}
    {\renewcommand{\arraystretch}{1.0}
    \begin{tabular}{|c|c|c|c|c|}
\toprule
\multicolumn{1}{c|}{Prompt Initialization Methods} & \multicolumn{1}{c|}{mIoU(S)} & \multicolumn{1}{c|}{\textbf{mIoU(U)}}  & \multicolumn{1}{c}{hIoU} \\ \hline
\multicolumn{1}{c|}{Shallow-random} & \multicolumn{1}{c|}{42.26} & \multicolumn{1}{c|}{37.43}    & \multicolumn{1}{c}{39.70} \\
\multicolumn{1}{c|}{Deep-random} & \multicolumn{1}{c|}{43.13} & \multicolumn{1}{c|}{40.5}    & \multicolumn{1}{c}{41.77} \\
\multicolumn{1}{c|}{Shallow-pretrain} & \multicolumn{1}{c|}{42.81} & \multicolumn{1}{c|}{42.40}    & \multicolumn{1}{c}{42.60} \\
\multicolumn{1}{c|}{Deep-pretrain} & \multicolumn{1}{c|}{\textbf{43.20}} & \multicolumn{1}{c|}{\textbf{45.02}}    & \multicolumn{1}{c}{\textbf{44.09}} \\
 \bottomrule
 \end{tabular}}}
}
\vspace{0.2em}
\caption{Ablation of different prompt initialization  strategies.}
\label{tab:prompt initialization}
\end{minipage}
\vspace{-2em}
\end{table}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  two tables
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{table}[!t]
\begin{minipage}{.49\linewidth}
\centering
\resizebox{\linewidth}{!}{{
\setlength{\tabcolsep}{0.5em}
    {\renewcommand{\arraystretch}{1.0}
    \begin{tabular}{|c|c|c|c|c|}
\toprule
\multicolumn{1}{c|}{Different Types of decoder} & \multicolumn{1}{c|}{mIoU(S)} & \multicolumn{1}{c|}{\textbf{mIoU(U)}}  & \multicolumn{1}{c}{hIoU} \\ \hline
\multicolumn{1}{c|}{Segmenter decoder~\cite{strudel2021segmenter}} & \multicolumn{1}{c|}{41.14} & \multicolumn{1}{c|}{40.41}    & \multicolumn{1}{c}{40.77} \\
\multicolumn{1}{c|}{SegViT decoder~\cite{zhang2022segvit}} & \multicolumn{1}{c|}{42.31} & \multicolumn{1}{c|}{42.02}    & \multicolumn{1}{c}{42.16} \\
\multicolumn{1}{c|}{Our decoder} & \multicolumn{1}{c|}{\textbf{43.20}} & \multicolumn{1}{c|}{\textbf{45.02}}    & \multicolumn{1}{c}{\textbf{44.09}} \\
 \bottomrule
 \end{tabular}
    }}}
\vspace{0.2em}
\caption{Analysis of different types of Decoder.}
\label{tab:decoder types}
\end{minipage}
\hspace{0.02\linewidth}
\begin{minipage}{.49\linewidth}
\centering

\resizebox{\linewidth}{!}{{
\setlength{\tabcolsep}{0.5em}
    {\renewcommand{\arraystretch}{1.0}
    \begin{tabular}{|c|c|c|c|c|}
\toprule
\multicolumn{1}{c|}{Class Weight Generator} & \multicolumn{1}{c|}{mIoU(S)} & \multicolumn{1}{c|}{\textbf{mIoU(U)}}  & \multicolumn{1}{c}{hIoU} \\ \hline
\multicolumn{1}{c|}{w/o} & \multicolumn{1}{c|}{43.07} & \multicolumn{1}{c|}{43.40}    & \multicolumn{1}{c}{43.23} \\
\multicolumn{1}{c|}{w} & \multicolumn{1}{c|}{\textbf{43.20}} & \multicolumn{1}{c|}{\textbf{45.02}}    & \multicolumn{1}{c}{\textbf{44.09}} \\

 \bottomrule
 \end{tabular}}}
}
\vspace{0.4em}
\caption{Ablation of class weight Generator}
\label{tab:prompt initialization}
\end{minipage}
\vspace{-1em}
\end{table}
\end{comment}







==> sections/Introduction.tex <==
\section{Introduction}

Semantic segmentation is a fundamental computer vision task that involves labeling each pixel in an image with a predefined class label. Limited to the labor-intensive pixel-level annotation, it is difficult to extend to a large number of object categories, especially to arbitrary categories.  In~\cite{bucher2019zero}, the setting of \textbf{Z}ero-\textbf{S}hot \textbf{S}emantic \textbf{S}egmentation (ZS3) is proposed to extend the capability of aligning pixels with predefined classes to unseen classes during the training phase.

%
Generative scheme \cite{bucher2019zero, li2020consistent} is the typical solution in the CNN era. Recently, the vision-language pre-trained models have been successfully applied to zero-shot semantic segmentation and achieved significant capability gain to segment unseen classes in a discriminative fashion~\cite{xu2022simple,ding2022decoupling,kim2023zegot,zhou2022zegclip}, where cross-attention based transformer is used as segment decoder to generalize the segmentation ability of seen classes to unseen classes. The language embedding is used as the query and the visual feature as the key and value in the cross-attention so that the semantic space is aligned with the visual space. In fact, the language embedding is sparse and distinct which is potential to compress the visual features to separable subspaces to increase the capacity of discrimination. 

Keeping the consistent relation of semantic space has been validated in the generative scheme~\cite{li2020consistent}. It is rarely considered in the cross-attention. In this paper, we propose a Semantic Compressed Visual Representation (SCVR) approach for zero-shot semantic segmentation, attempting to compress the visual feature by the constraint of language embedding in visual space and force them to compact subspace to increase the discrimination, as shown in Fig.~\ref{fig:motivation}. It is carried out with simple-yet-effective Semantic Compressed Cross-attention (SCC), where the visual feature is input as the query, and the language embedding is used as the key and value. The cross-attention mechanism in the transformer updates the query based on the similarity of the query and the key, so that the visual embedding is forced to increase the similarity with the embedding of class names in SCC, $i.e.$, approaching the projection of class category within the visual space. 

With SCVR, the text embedding is updated slightly compared with the previous segment decoder \cite{zhang2022segvit,strudel2021segmenter,zhou2022zegclip}. To make the text embedding learnable, both vision prompt learning and language prompt learning are utilized. The vision prompt follows the deep prompting learning~\cite{jia2022visual}. The deep architecture is also applied to language prompt tuning, in which the learnable prompts are inserted to shallow and deep layers. We observe that it's awesome to initialize deep language prompts with hidden features, which are generated by the CLIP language encoder with the input of templates, $e.g.$, ``a photo of a".
% 
With deep vision-language prompt tuning, SCVR further improves the segmentation performance both on seen and unseen classes.

We conduct experiments on the two public PASCAL VOC 2012 and COCO-Stuff 164k datasets. Compared with the previous segment decoder, the visualization of visual features clearly exhibits that they are compressed. The experimental results show that our approach outperforms the SOTA method by 0.6\% of seen classes and 4.5\% of unseen classes on PASCAL VOC 2012 dataset, 3.0\% and 3.6\% on COCO-Stuff 164k dataset, respectively. 

The main contributions are summarized as follows:
\begin{enumerate}
    \item A semantic compressed cross-attention module is proposed to enhance the segment decoder, which aggregates visual features to distinguishable subspaces with higher discrimination capacity.
    \item A vision-language prompt tuning strategy is proposed to generalize the pre-trained CLIP to zero-shot semantic segmentation, which further improves unseen classes segmentation ability.
    %    
    \item Extensive experiments and visualization validate the ability of semantic compressed cross-attention and illustrate significant gain of semantic segmentation performance on both seen and unseen classes.
\end{enumerate}



\begin{figure}[!t]
\centering
    \includegraphics[width=0.99\textwidth]{imgs/mechanism.pdf}
\vspace{-1em}
\caption{The diagram illustrates, from left to right, the changes in visual space as the image passes through our model's pipeline, along with the underlying mechanism of these updates. In the first stage, the visual space from encoder is not disentangled and structured enough, on sides of the classification boundary, there exist many misclassified visual features. In the second stage, we leverage cross-attention mechanism to use class embeddings (acting as value and key) to force the visual features (acting as query) approach their corresponding class embedding, which makes visual features more semantic compressed and leads to a disentangled visual space shown in the third stage.}
\vspace{-1em}
\label{fig:motivation}
\end{figure}
\begin{comment}

\begin{figure}[!t]

\centering
    \includegraphics[width=0.98\textwidth]{imgs/introduction_old.pdf}
\vspace{0.5em}
\caption{Arch}
\label{fig:introduction_new}
\end{figure}
\end{comment}

==> sections/Method.tex <==
\section{Methodology}


%  arch image
\begin{figure}[!t]
\centering
        \includegraphics[width=0.98\textwidth]{imgs/arch_new.pdf}
% \vspace{-0.5em}
\caption{The architecture of our method. We freeze the parameters of CLIP and insert deep learnable visual-language prompts into encoders. Then a text adapter fuses text embeddings $T$ and global image feature $V_g$. At last, SCVR decoder compresses the dense visual features $V_l$ under the guide of updated text embeddings $T_{new}$ to get the segmentation logits $S$.}
\vspace{-1em}
\label{fig:arch}

\end{figure}

\subsection{Overview}
Our proposed method follows the generalized zero-shot semantic segmentation(GZS3) protocol~\cite{xian2019semantic}. The protocol divides the class set into two disjoint subsets: seen class set $C^s$ and unseen class set $C^u$. The model training is conducted only on $C^s$ while evaluation on both $C^s$ and $C^u$. Specifically, during the training phase, we only have pixel-wise annotations about $C^s$ on each image. During the inference phase, we need to classify each pixel of the image as one of the classes in $C=C^u \cup C^s$. 
Inductive ZS3 setting
% ~\cite{ding2022decoupling} 
aims to solve the case that unseen class names are not known during training. In contrast, the unseen class names are specified in the transductive ZS3 setting.
% ~\cite{kim2023zegot} 
We use 'inductive' settings following~\cite{ding2022decoupling} as it can better demonstrate the model generalization on unseen classes.

The overall architecture of our proposed method is illustrated in Fig.~\ref{fig:arch} with the one-stage paradigm. In the encoder part, we freeze the parameters of both text and image encoders of the pre-trained CLIP, and insert both visual and language prompts into each layer of them. Then a text adapter module fuses the text embedding $T$ from the text encoder and the global image embedding. $V_g$ from the image encoder. At last, the proposed SCVR decoder compresses the visual representation constrained by the text adapter and outputs the prediction of semantic segmentation. 
% % Besides we design a class weight generator module to dynamically scale the class-wise segment logits.


\subsection{SCVR Decoder}
Given an image $I\in \mathbb{R}^{H\times W \times 3}$ and class sets $C$, the CLIP encoders with visual-language prompts output dense image feature $V_l\in \mathbb{R}^{h\times w\times d}$,
multi-intermediate image features $\{V_j\}_{j=1,2,\dots,N}$, 
global image feature $V_g\in \mathbb{R}^{d}$ (corresponding to [CLS] token), and text embeddings of class names $T \in \mathbb{R}^{c\times d}$, where $h$ and $w$ are the height and width of dense image features respectively, $d$ is the dimension of the CLIP's joint embedding space, $c$ is the number of semantic categories, and $N$ is the number of decoder layers. 

\textbf{Text Adapter.} Following the design of previous methods~\cite{kim2023zegot,zhou2022zegclip}, we utilize a text adapter to fuse $V_g$ and $T$ to inject visual information into text embeddings. The text adapter is implemented as:
\begin{align}
    T_{\mathrm{new}} = \mathbf{Proj}([T \odot V_g; T ]),
\end{align}
where $\mathbf{Proj}$ is a linear projection, $\odot$ represents broadcast element-wise multiplication \rebuttal{and $[;]$ represents concatenation operation of tensors}. The fused text embeddings $T_{\mathrm{new}}\in \mathbb{R}^{c\times d}$ have the same size as $T$, which is inputted as key-value to the SCVR decoder. 

\textbf{Decoder.}
Segmentation decoder essentially functions as a clustering mechanism that aggregates the high-level dense features into the class-wise partition. To increase the classification ability of the decoder, it's natural to compress the dense feature to compact partitions.
As demonstrated in previous works~\cite{yu2022cmt,yu2022k}, cross attention is equivalent to \textit{k}-means~\cite{hartigan1979algorithm} with a soft assignment. It motivates us to force the visual features to be close to the unique semantic center, \textit{i.e.}, embedding of the class name, with semantic compressed cross-attention (SCC). 

Based on SCC, the transformer-like SCVR decoder block is proposed, which is stacked to predict the semantic segmentation, as shown in Fig. \ref{fig:arch}.
% Thus we design an attention-based decoder to align the high-level dense features with class embeddings from CLIP. 
Supposing $V_{in}$ and $V_{out}$ are the input and output of the decoder block, 
it is accomplished as:
% The overall of our decoder block can be summarized as follow:
\begin{align}
V & = V_{in} + \mathbf{LocalAttn}(\mathbf{Norm}(V_{in})) \\
V & = V + \mathbf{CrossAttn}(\mathbf{Norm}(V),\mathbf{Norm}(T_{\mathrm{new}})) \\
V_{out} & = V +\mathbf{MLP}(\mathbf{Norm}(V)),
\end{align}
where $\mathbf{Conv}$ is a convolution layer with 1$\times$1 kernel, $\mathbf{Norm}$ is layer normalization~\cite{ba2016layer}, $\mathbf{LocalAttn}$ is local self-attention,  $\mathbf{CrossAttn}$ is the standard cross attention operation, and $\mathbf{MLP}$ is a layer of multi-layer perception. It's worth mentioning that the $V_{in}$ integrates the intermediate image features of CLIP encoder, computed as:
\begin{align}
V_{in} & = V_{init} + \mathbf{Conv}(V_{\delta(\cdot)}) 
\end{align}
where $V_{init}$ is set as $V_l$ for the first decoder block and the output of the former one for the stacked blocks, $\delta( \cdot ) \in \{j=1,2,\dots,N\}$ is a selection function to choose the intermediate feature of CLIP \footnote{The selection strategy is discussed in the supplementary material. }.   

% and represents the output of the (j$-$1)-th block, and the initial $V$ is $V_l$. .

%The differences between our decoder and other query-based transformer decoders like SegViT~\cite{zhang2022segvit} and mask2former~\cite{cheng2022masked} lies in two aspects:
%1) our query is dense image features and our key and value are class embeddings. We use class embeddings as condition to update image features. 2) We substitute standard self attention with a special local self attention which can aggregate local context information to update dense image features.
The design of $\mathbf{LocalAttn}$ follows BiFormer~\cite{zhu2023biformer}. For dense image features $V_{in}$, we first employ an average pooling layer with a window size of $n\times n$ to extract window features $V_w\in \mathbb{R}^{h/n\times w/n \times d}$. Then we calculate the similarity between each window feature and choose $m$ windows that are most relevant for each window feature. Based on the routing, we constrain self-attention for $V_{in}$ in the selected $m$ windows. The operations are as follows
\begin{align}
    V_w & = \mathbf{AvgPool}(V_{in}) \\
    Q,K,V & = \mathbf{Chunk}(\mathbf{Proj}(V_{in})) \\
    \mathrm{ids} & = \mathbf{Topk}(V_w V_w^T,m) \\
    K_{gather}, V_{gather} &= \mathbf{Gather}(K,\mathrm{ids}), \mathbf{Gather}(V,\mathrm{ids}) \\
    V &= \mathbf{Softmax}(QK_{gather}^T/\sqrt{d}) V_{gather},
\end{align}
where $\mathbf{AvgPool}$ denotes average pooling operation, $\mathbf{Proj}$ denotes linear projection which projects $V_{in}$ from length $d$ to $3d$, $\mathbf{Chunk}$ means splitting the tensor along the last dimension, $\mathbf{Topk}$ returns the indices of $m$-largest elements of given tensor, $\mathbf{Gather}$ denotes the operation that gathers tensor according to indices, and $\mathbf{Softmax}$ denotes a softmax layer. 

Finally, forward several stacked decoder blocks, we get the final image feature $V_o\in \mathbb{R}^{h\times w \times d}$ and we multiply $V_o$ with $T_{\mathrm{new}}$ to produce segmentation logits $S\in \mathbb{R}^{c\times h \times w}$, as:
\begin{align}
    S =  T_{\mathrm{new}} V_o^T.
\end{align}

% \noindent\textbf{Class Weight Generator.} For a given image, it only contains several categories from the class set. Thus we design a class weight generator to dynamically scale the class-wise segment logits $S$, which amplifies the classes occurred in image and suppresses the other classes. Specifically, we utilize cross attention blocks to align $T_{\mathrm{new}}$ with $V_l$ and calculate the similarity between the updated $T_{\mathrm{new}}$ and $V_g$ as class-wise scale weights $W_c\in \mathbb{R}^{c}$. The details of cross attention blocks are as follow:
% \begin{align}
%     T'&= T_{\mathrm{new}} + \mathbf{CrossAttn}(\mathbf{Norm}(T_{\mathrm{new}}),\mathbf{Norm}(V_l)) \\
%     T'_{\mathrm{new}} &=  T'+ \mathbf{MLP}(\mathbf{Norm}(T')).
% \end{align}
% The process of generating $W_c$ and final segmentation logits $S_f\in \mathbb{R}^{c\times h \times w}$ is as follows:
% \begin{align}
%     W_c &= T'_{\mathrm{new}} V_g \\
%     S_f &= S * W_c. 
% \end{align}
\subsection{Visual-Language Prompt Tuning}

\noindent\textbf{Visual Prompt Tuning. }
As mentioned in ZegCLIP~\cite{zhou2022zegclip}, compared to full fine-tuning and parameter-free fine-tuning, deep visual prompt tuning~\cite{jia2022visual} can achieve a trade-off between segmentation performance and zero-shot capabilities. We equip the CLIP image encoder  with the same structure as ZegCLIP. Moreover, we find that introducing deep prompt tuning in the CLIP text encoder with elaborate design can further enhance the zero-shot segmentation capabilities. 
% We first briefly introduce the CLIP text encoder and then introduce how to leverage deep prompt tuning to fine-tune it.

\noindent\textbf{Language Prompt Tuning. }
% \noindent\textbf{CLIP Text Encoder.} 
The text encoder of CLIP is based on transformer~\cite{vaswani2017attention}. 
We divide the input text \textit{“a photo of a \{class name\}.”} to context text \textit{"a photo of a"} and class text \textit{"{class name}"}.
% Given the input text like \textit{“a photo of a \{class name\}.”}, we divide it into two parts: context text and class text. The context text refers to the text \textit{"a photo of a"} and the class text refers to the text \textit{"{class name}"}. 
The tokenizer of CLIP tokenizes the text into text tokens and maps them to discrete numbers according to the predefined dictionary~\cite{sennrich2015neural}. 
By bracketing the text tokens with \textrm{[SOS]} and \textrm{[EOS]}, CLIP projects text tokens to text embeddings $E^{(0)}$.
% Besides the tokenizer will bracket the text tokens with \textrm{[SOS]} and \textrm{[EOS]}. Then the embedding layer of CLIP will project text tokens to text embeddings $E^{(0)}$. 
According to the partition of text token, the $E^{(0)}$ is formulated as:
\begin{align}
E^{(0)}=[E^{(0)}_{\textrm{s}};E^{(0)}_{\textrm{context}};E^{(0)}_{\textrm{class}};E^{(0)}_{\textrm{e}}],
\end{align}
where $E^{(0)}_{\textrm{s}}$, $E^{(0)}_{\textrm{context}}$, $E^{(0)}_{\textrm{class}}$, $E^{(0)}_{\textrm{e}}$ represent the embeddings of [SOS] token, context token, class token, and [EOS] token respectively, and ";" represents concatenation operator. 
% After that the transformer encoder with $l$ layers will process the $E^{(0)}$ and produce the final text feature $z$. The process is as follow:
The embedding $E^{(0)}$ is passed through transformer encoder with $l$ layers to produce the final text feature $z$, as:
\begin{align}
E^{(i)} &= \mathbf{L}_{i} ([E^{(i-1)}_{\textrm{s}};E^{(i-1)}_{\textrm{context}};E^{(i-1)}_{\textrm{class}};E^{(i-1)}_{\textrm{e}}]) \quad\quad i = 1,2,3,\dots,l  \\
E_z &= \mathbf{Head}(E^{(l)}_{\textrm{e}}),
\end{align}
where $\mathbf{L}_{i}$ denotes $i$-th layer of transformer encoder and $\mathbf{Head}$ denotes the final projection. After normalization, $E_z$ is used to match the global image feature $V_g$ from the CLIP image encoder.

% \noindent\textbf{Language Deep Prompt Tuning.} 
Similar to the design of VPT~\cite{jia2022visual}, we replace $E^{(i)}_{\textrm{context}}$al by learnable prompts $\mathcal{P}^{(i)}$ for each layer and freeze the parameters in $\mathbf{L}_{i}$. The forward approach is updated as:
\begin{align}
[E^{(i)}_{\textrm{s}};\_;E^{(i)}_{\textrm{class}};E^{(i)}_{\textrm{e}}] &= \mathbf{L}_{i} ([E^{(i-1)}_{\textrm{s}};\mathcal{P}^{(i-1)};E^{(i-1)}_{\textrm{class}};E^{(i-1)}_{\textrm{e}}]) \quad\quad i = 1,2,3,\dots,l  \\
z &= \mathbf{Head}(E^{(l)}_{\textrm{e}}).
\end{align}
The key factor lies in how to \textbf{initialize} $\mathcal{P}^{(i)}$. As $\mathcal{P}^{(i)}$  replaces the $E^{(i)}_{\textrm{context}}$, it's initialized
% We replace $E^{(i)}_{\textrm{context}}$ by $\mathcal{P}^{(i)}$, so we initialize $\mathcal{P}^{(i)}$ 
by the value of $E^{(i)}_{\textrm{context}}$ rather than sample 
 from a random distribution.
 % . We discuss this design in Tab. ~\ref{tab:prompt initialization}.
With the design of language deep prompt tuning, we combine it with visual deep prompt tuning to efficiently fine-tune CLIP encoders as shown in fig.~\ref{fig:arch}. \label{par:initialization}

\subsection{Discussion}
\label{section:discussions}
According to information bottleneck theory~\cite{michael2018on,shwartz2017opening}, a good feature should compress the input as much as possible while maximizing mutual information with the output. The visual space from the pre-trained backbone is usually not disentangled and structured enough for segmentation due to the mismatch between upstream and downstream tasks. Under full supervision, the model utilizes gradients to implicitly update and structure the original visual space. Under ZS3 settings, prompt tuning~\cite{zhou2022zegclip} and parameter-free fine-tuning~\cite{kim2023zegot} were validated outperforming full fine-tuning. However, it implies that the flexibility is reduced in updating the visual space. In this paper, we utilize visual features as the query to explicitly update visual space, providing a simple-yet-effective way to conquer this drawback. \label{par:explicit update}



==> sections/Related.tex <==
\section{Related Work}

\noindent\textbf{Zero-Shot Semantic Segmentation.}
% Semantic segmentation is a fundamental computer vision task that involves labeling each pixel in an image with a corresponding predefined class label. Zero-shot semantic segmentation(ZS3) aims to extend the capability of aligning pixels with predefined classes to novel classes which don't appear during the training phase. 
The setting of Zero-Shot Semantic Segmentation is proposed in~\cite{bucher2019zero}. The typical methods~\cite{bucher2019zero,li2020consistent,gu2020context} use generative models to transform unseen classes text embeddings into dense visual features. Though effective, these methods exhibit suboptimal performance on unseen classes due to the lack of prior knowledge. With the advent of vision-language pre-trained models~\cite{radford2021learning,jia2021scaling}, the core concerns about this task shift into how to transfer zero-shot learning capabilities from image-level to pixel-level. On this basis, recent works derive two streamlines: the two-stage method and the one-stage method. Two-stage methods~\cite{xu2022simple,ding2022decoupling} decouple the task into two phases, in which class-agnostic masks are generated first and a zero-shot classifier assign the masks with labels. As the former training phase is class-agnostic, it can be directly transferred to generate unseen class masks. The latter phase leverages the  CLIP's~\cite{radford2021learning} image-level zero-shot capabilities to classify the masks. Although it well maintains the zero-shot capabilities of CLIP, the inference cost is heavy due to the separate classification of the huge amount of masks per image. The one-stage methods~\cite{kim2023zegot,zhou2022zegclip,xu2023side,rao2022denseclip} directly optimize CLIP's backbones to transfer the zero-shot capabilities from image-level to pixel-level. The one-stage methods are with better performance and less inference cost. However, it lacks exploring the potential of the spare and distinct embeddings of class names. We follow the paradigm of the one-stage and further compress the visual feature guided by the semantic language embedding to increase the classification ability of the segment decoder.
% Our method follows the paradigm of the one-stage method and further enhances the performance of one-stage methods.

\noindent\textbf{Prompt Tuning.}
Prompt tuning was first introduced in natural language processing~\cite{brown2020language} which fixes the parameters of the pre-trained model and inserts a small set of learnable parameters to adapt the pre-trained model to downstream tasks. Prompt tuning methods maintain the generalization ability of the pre-trained model while adapting well to downstream tasks. Recently, many works introduce prompt tuning to \rebuttal{computer} vision and discuss it in the image recognition task.
% The approaches can be divided into three aspects: 1) vision-only prompt tuning, 2) language-only prompt tuning, and 3) vision-language prompt tuning. 
Vision-only prompt tuning mainly focuses on parameter-efficient tuning about ViT~\cite{dosovitskiy2020image}. VPT~\cite{jia2022visual} was the first work to leverage prompt tuning to fine-tune ViT, which inserts learnable prompts between [CLS] token and visual patch tokens in each transformer~\cite{vaswani2017attention} block. EXPRES~\cite{das2023learning} improves VPT by adding residual learnable tokens to reweight the attention maps. Language-only prompt tuning focuses on optimizing downstream text prompts close to the format of upstream natural texts. CoOp~\cite{zhou2022learning} first introduced learnable prompts in text embeddings. Further, CoCoOp~\cite{zhou2022conditional} and DenseCLIP~\cite{rao2022denseclip} use image features to condition learnable prompts for better adaption. Vision-Language prompt tuning was recently introduced by MaPLe~\cite{khattak2022maple}, which inserts learnable prompts in both the visual encoder and the text encoder and leverages text prompts to guide visual prompts. We follow the paradigm of vision-language prompt tuning and insert deep independent learnable prompts in both visual and text encoders. Besides we design a special initialization strategy for language prompts.

\noindent\textbf{Decoder for Plain ViT.}
Although hierarchical ViTs~\cite{liu2021swin,zhu2023biformer} is a more powerful backbone by introducing visual inductive bias, plain ViT~\cite{dosovitskiy2020image} still possesses irreplaceable advantages, as Plain ViT scales well with huge data and Plain ViT can easily introduce the latest self-supervised techniques like MAE~\cite{he2022masked} and BEiT~\cite{bao2021beit}. Many foundation models, like CLIP~\cite{das2023learning} and SAM~\cite{kirillov2023segment}, still adopt plain ViT as their image encoders. Therefore, quite a lot of approaches have tried to design a decoder suitable for plain ViT. 

SETR~\cite{zheng2021rethinking} and DPT~\cite{ranftl2021vision} design a CNN-based decoder for plain ViT. Segmenter~\cite{strudel2021segmenter} equips plain ViT with a lightweight transformer based decoder and uses self-attention to joint process learnable class embeddings and image patches. ViT-Adapter~\cite{chen2022vision} utilizes adapters to produce hierarchical features for plain ViT and adapts it for previous FPN-like~\cite{lin2017feature} decoders. Inspired by Maskformer~\cite{cheng2021per}, SegViT~\cite{zhang2022segvit} leverages the cross-attention maps of class embeddings and image patches to generate mask predictions for each category, which alleviates the need for FPN-like pixel decoder in Maskformer. The above methods are all designed for the task of semantic segmentation. In ZS3, the decoder design is often ignored. for example, ZegFormer~\cite{ding2022decoupling} adopts Maskformer decoder without modification and ZegCLIP~\cite{zhou2022zegclip} adopts SegViT decoder directly. We propose a new decoder for ZS3 with the architecture of the transformer block. It consists of local attention to aggregate local context and a semantic compressed cross-attention to force the visual features to distinguish subspace. 

The most similar cross-attention mechanism is proposed in~\cite{rombach2022high}, in which a text-conditioned cross-attention is used for conditional image generation. In ~\cite{rombach2022high}, language embedding is utilized to control local contents of image. In this paper, we use the semantic information of language embedding to compress the visual features for discriminative representation. These two works show the effectiveness of text-conditioned cross-attention on both generative and discriminative tasks.

% {\color{red}Considering the characteristic of ZS3 backbone being more suitable for prompt tuning and parameter-free fine-tuning, we designed a decoder that is more appropriate for ZS3.}
